iDRM: Humanoid Motion Planning with Real-Time End-Pose Selection in Complex Environments

In this paper, we propose a novel inverse Dynamic Reachability Map (iDRM) that allows a floating base system to find valid end-poses in complex and dynamically changing environments in real-time. End-pose planning for valid stance pose and collision-free configuration is an essential problem for humanoid applications, such as providing goal states for walking and motion planners. However, this is non-trivial in complex environments, where standing locations and reaching postures are restricted by obstacles. Our proposed iDRM customizes the robot-to-workspace occupation list and uses an online update algorithm to enable efficient reconstruction of the reachability map to guarantee that the selected end-poses are always collision-free. The iDRM was evaluated in a variety of reaching tasks using the 38 degree-of-freedom (DoF) humanoid robot Valkyrie. Our results show that the approach is capable of finding valid end-poses in a fraction of a second. Significantly, we also demonstrate that motion planning algorithms integrating our end-pose planning method are more efficient than those not utilizing this technique.

==> setup.tex <==
\newcommand{\myTitle}{iDRM: Humanoid Motion Planning with Real--Time End--Pose Selection in Complex Environments}
\newcommand{\myName}{Yiming Yang, Vladimir Ivan, Zhibin Li, Maurice Fallon, Sethu Vijayakumar}
\newcommand{\myDepartment}{School of Informatics}
\newcommand{\myUni}{University of Edinburgh}

\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}

\usepackage{multicol}
\usepackage{amsmath}
\usepackage{etoolbox}
\usepackage{capt-of}
\usepackage[noend]{algpseudocode}
\usepackage{amssymb}
\usepackage{subfig}
%\usepackage{caption}
%\usepackage{subcaption}
\usepackage{soul}
\usepackage{color}
\usepackage{multirow}
\usepackage{makecell}

\PassOptionsToPackage{dvipsnames}{xcolor}
	\RequirePackage{xcolor} % [dvipsnames] 
\definecolor{halfgray}{gray}{0.55} % chapter numbers will be semi transparent .5 .55 .6 .0
\definecolor{webgreen}{rgb}{0,.5,0}
\definecolor{webbrown}{rgb}{.5,0,0}
\definecolor{Maroon}{cmyk}{0, 0.87, 0.68, 0.32}
\definecolor{RoyalBlue}{cmyk}{1, 0.50, 0, 0}
\definecolor{Black}{cmyk}{0, 0, 0, 0}

\usepackage{float}
\PassOptionsToPackage{pdftex,hyperfootnotes=false,pdfpagelabels}{hyperref}
\usepackage{hyperref}
\pdfcompresslevel=9
\pdfadjustspacing=1 
\PassOptionsToPackage{pdftex}{graphicx}
	\usepackage{graphicx} 
	
\hypersetup{%
     %draft,	% = no hyperlinking at all (useful in b/w printouts)
     colorlinks=true, linktocpage=true, pdfstartpage=3, pdfstartview=FitV,%
     % uncomment the following line if you want to have black links (e.g., for printing)
     %colorlinks=false, linktocpage=false, pdfborder={0 0 0}, pdfstartpage=3, pdfstartview=FitV,% 
     breaklinks=true, pdfpagemode=UseNone, pageanchor=true, pdfpagemode=UseOutlines,%
     plainpages=false, bookmarksnumbered, bookmarksopen=true, bookmarksopenlevel=1,%
     hypertexnames=true, pdfhighlight=/O,%nesting=true,%frenchlinks,%
     urlcolor=webbrown, linkcolor=RoyalBlue, citecolor=webgreen, %pagecolor=RoyalBlue,%
     pdftitle={\myTitle},%
     pdfauthor={\textcopyright\ \myName, \myUni, \myDepartment},%
     pdfsubject={},%
     pdfkeywords={},%
     pdfcreator={pdfLaTeX},%
     pdfproducer={LaTeX with hyperref and classicthesis},%
} 
